Simulation-to-Real domain adaptation with teacher-student learning for endoscopic instrument segmentation

Purpose: Segmentation of surgical instruments in endoscopic videos is essential for automated surgical scene understanding and process modeling. However, relying on fully supervised deep learning for this task is challenging because manual annotation occupies valuable time of the clinical experts. Methods: We introduce a teacher-student learning approach that learns jointly from annotated simulation data and unlabeled real data to tackle the erroneous learning problem of the current consistency-based unsupervised domain adaptation framework. Results: Empirical results on three datasets highlight the effectiveness of the proposed framework over current approaches for the endoscopic instrument segmentation task. Additionally, we provide analysis of major factors affecting the performance on all datasets to highlight the strengths and failure modes of our approach. Conclusion: We show that our proposed approach can successfully exploit the unlabeled real endoscopic video frames and improve generalization performance over pure simulation-based training and the previous state-of-the-art. This takes us one step closer to effective segmentation of surgical tools in the annotation scarce setting.

==> Sections/DomainAdaptation.tex <==
% TL -> DA -> Deep UDA
Domain Adaptation (DA) is a scenario of \textit{transfer learning \cite{tan2018surveytl}} where the source and target tasks are similar, however, the source and target domains are different. DA can be further categorized into three sub-categories: supervised DA, semi-supervised DA and unsupervised DA as per the level of supervision required on the target domain.
Authors would like to direct readers to the survey articles \cite{wang2018surveyda} and \cite{wilson2020surveyuda,zhao2020review} for domain adaptation and unsupervised domain adaptation literature.
Types: discrepancy-baased \cite{long2015learning}, adversial-based \cite{ganin2016domain,hoffman2016fcns,shrivastava2017learning,hoffman2018cycada}, self-training \cite{french2018self} , curriculum-learning \cite{sakaridis2018model} or combinations 
% In contrast to adversial based appraoch, we focussed on self-training appraoch 



==> Tables/Comparison_Work.tex <==
%\begingroup
%\begin{table}[htbp] 
%\centering
%\setlength{\tabcolsep}{6pt} %space between columns
%\renewcommand{\arraystretch}{1.0} %space between rows
% table caption is above the table
%\captionsetup{justification=centering}
\begin{tabular}{ c  c  c  c }
%\begin{tabular}{| c | c | c | c |}
	\hline\noalign{\smallskip}
	%\hline
	Approach & Source (L$|$UL) & Target (L$|$UL) & Domain Adaptation (Steps) \\
	\noalign{\smallskip}\hline\noalign{\smallskip}
	%\hline
	%\hline
	PAT ~\cite{ross2018exploiting} & Real (L) & Real (L) & Semi-supervised (Two-step) \\
	I2I ~\cite{pfeiffer2019generating} & Simulated (L) & Real (UL) & Unsupervised (Two-step) \\
	\noalign{\smallskip}\hline\noalign{\smallskip}
	%\hline 
	Ours & Simulated (L) & Real (UL) & Unsupervised (End-to-end) \\
	\noalign{\smallskip}\hline
	%\hline
\end{tabular}
%\end{table}
%\begingroup

==> Tables/Comparisons.tex <==
\begingroup	
    % table 1
    \begin{subtable}{.5 \linewidth}
    \centering
    \caption{Endo-Sim2Real~\cite{sahu2020endo}} \label{table:Result_Compare:CL}
    \setlength{\tabcolsep}{3pt}
        \begin{tabular}{| l | c | c |}
	    	\hline
	    	$T$/$Loss$ & MSE & S-CL \\
	    	\hline 
	    	\hline
	    	Weak    & .50  & .69\\ 
	    	Strong  & .41  & .73\\
	    	\hline
	    \end{tabular}
	\end{subtable} %
    % table 2
	\begin{subtable}{.5 \linewidth}
	\centering
    \caption{Endo-Sim2Real (Teacher-Student)}
    \label{table:Result_Compare:I2I}
    \setlength{\tabcolsep}{3pt}
    	\begin{tabular}{| l | c | c |}
    		\hline
    		$T$/$Loss$ & MSE & S-CL \\
    		\hline 
    		\hline
    		Weak    & .35           & \textbf{.75}\\ 
	    	Strong  & \textbf{.44}  & \textbf{.80}\\
    		\hline
    	\end{tabular}
	\end{subtable} %
\endgroup

==> Tables/Dice_Distributions.tex <==
\begin{comment}
% For two-column wide figures use figure*
% using subfigure or minipage
\begin{figure*}[t]
	%
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/endovis.pdf}
        \caption{EndoVis (0 \% empty)}
        \label{fig:dice_distribution_endovis}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/cholec.pdf}
        \caption{Cholec (13 \% empty)}
        % NoTool: 278, SB: 12, NaN: 110, Empty FP: 180 (8.43 \%)
        \label{fig:dice_distribution_cholec}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Figures/robustmis.pdf}
        \caption{RobustMIS (20 \% empty)}
        % NoTool: 818, NaN: 389, Empty FP: 429 (10.6 \%)
        \label{fig:dice_distribution_robustmis}
    \end{subfigure}
    % figure caption is below the figure
    \caption{Dice distribution across datasets (Best viewed in color with 200 \% zoom)}
	\label{fig:dice_distribution}
\end{figure*}
\end{comment}

\begin{comment}
% For two-column wide figures use figure*
% using subfigure or minipage
\begin{figure*}
	%
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{Figures/dice_boxplot.png}
        \caption{Dice Histogram}
        \label{fig:Dice_Histogram}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{Figures/histplot.pdf}
        \caption{Dice distribution}
        \label{fig:dice_distribution}
    \end{subfigure}
    % figure caption is below the figure
    \caption{Per tool statistics}% (Best viewed in color with 200 \% zoom)}
	\label{fig:Stats_per_tool}
\end{figure*}
\end{comment}
